Asymmetric Variational Autoencoders

Variational inference for latent variable models is prevalent in various machine learning problems, typically solved by maximizing the Evidence Lower Bound (ELBO) of the true data likelihood with respect to a variational distribution. However, freely enriching the family of variational distribution is challenging since the ELBO requires variational likelihood evaluations of the latent variables. In this paper, we propose a novel framework to enrich the variational family by incorporating auxiliary variables to the variational family. The resulting inference network doesn't require density evaluations for the auxiliary variables and thus complex implicit densities over the auxiliary variables can be constructed by neural networks. It can be shown that the actual variational posterior of the proposed approach is essentially modeling a rich probabilistic mixture of simple variational posterior indexed by auxiliary variables, thus a flexible inference model can be built. Empirical evaluations on several density estimation tasks demonstrates the effectiveness of the proposed method.

==> body.tex <==
\begin{abstract}

  Bayesian posterior inference is prevalent in various machine
  learning problems. Variational inference provides one way to
  approximate the posterior distribution, however its expressive power
  is limited and so is the accuracy of resulting
  approximation. Recently, there has a trend of using neural networks
  to approximate the posterior distribution given the flexibility and
  coverage of neural network models. However, previous models strongly
  restrict the structure of the network in favor of computational
  efficiency. In this paper, we propose a new family of neural network
  models to approximate the posterior distribution... Experiments on
  synthetic and real world posterior inference problems demonstrate
  the effectiveness and efficiency of the proposed method.

\end{abstract}

\section{INTRODUCTION}

Posterior inference is the key to Bayesian modeling, where we are
interested to see how our belief over the variables of interest change
after observing a set of data points. Predictions can also benefit
from Bayesian modeling as every prediction will be equipped with
confidence intervals representing how sure the prediction is. Compared
to the maximum a posteriori estimator of the model parameters, which
is a point estimator, the posterior distribution provide richer
information about the model parameter hence enabling more justified
prediction.

Among the various inference algorithms for posterior estimation,
variational inference (VI) and Monte Carlo Markov chain (MCMC) are the
most two wisely used ones. It is well known that MCMC suffers from
slow mixing time though asymptotically the samples from the chain will
be distributed from the true posterior. VI, on the other hand,
facilitates faster inference, since it is optimizing an explicit
objective function and convergence can be measured and controlled, and
it's been widely used in many Bayesian models, such as Latent
Dirichlet Allocation \cite{DBLP:journals/jmlr/BleiNJ03}, etc. However,
one drawback of VI is that it makes strong assumption about the shape
of the posterior such as the posterior can be decomposed into multiple
independent factors. Though faster convergence can be achieved by
paramater learning, the approximating accuracy is largely limited.

The above drawbacks stimulates the interest for richer function
families to approximate posteriors while maintaining acceptable
learning spped. Specifically, neural network is one among such models
which has large modeling capacity and endows efficient
learning. \cite{DBLP:conf/icml/RezendeM15} proposed normalization
flow, where the neural network is set up to learn an invertible
transformation from one known distribution, which is easy to sample
from, to the true posterior. Model learning is achieved by minimizing
the KL divergence between the empirical distribution of the generated
samples and the true posterior. After propoerly trained, the model
will generate samples which are close to the true posterior, so that
Bayesian predictions are made possible. Other methods based on
modeling random variable transformation, but based on different
formulations are also explored. The Inverse Autoregressive Flow
\cite{DBLP:journals/corr/KingmaSW16} models the transformation as operations among the different
dimensions of the random variable. Though these methods greatly
increase the capacity of the distributions they can approximate, they
still suffer from the following two drawbacks:

\begin{itemize}
\item They make over simplied use of the neural network structure, and
  in order to achieve a ceterain degree of approximating accuracy,
  more layers of stacking up the basic unit is needed;
\item One key component in the modeling is computing the determinant
  of the Jacobian of the transformation, and in order to facilitate
  efficient learning, only very simple functions are used.
\end{itemize}

To address the above two factors, we propose a new unit to transform
the random variables...

The remainder of this paper is organized as follows....

\section{PRELIMINARIES}

\subsection{Transformation of random variables}

Given random variable $\vect z\in\mathbb{R}^d$ with density $p(\vect
z)$, consider a smooth and invertible function
$f:\mathbb{R}^d\rightarrow\mathbb{R}^d$ operated on $\vect z$. Let
$\vect z'=f(\vect z)$ be the resulting random variable, hence the
density of $\vect z'$ is
\begin{align}
  p(\vect z')=p(z)\left|\det \frac{\partial f^{-1}}{\partial \vect z'}\right|=p(z)\left|\det \frac{\partial f}{\partial \vect z}\right|^{-1}
\end{align}

 \subsection{Normalizing flows}
 
Normalizing flows considers successively transforming $\vect z_0$ with a
series of transformations $\{f_1, f_2, ..., f_K\}$ to construct
arbitrarily complex densities for $\vect z_K=f_K\circ f_{K-1}\circ...\circ f_1(\vect z_0)$ as
\begin{align}
  \log p(\vect z_K)=\log p(\vect z_0)-\sum_{k=1}^K\log\left|\det \frac{\partial f_k}{\partial \vect z_{k-1}}\right|
\end{align}

Hence the complexity lies in computing the determinant of the Jacobian
matrix. Without further assumption about $f$, the general complexity
for that is $\mathcal{O}(d^3)$ where $d$ is the dimension of $\vect
z$. In order to accelerate this, \cite{DBLP:conf/icml/RezendeM15} proposed the following family
of transformations that they termed as \textit{planar flow}:
\begin{align}
  f(\vect z)=\vect z+\vect uh(\vect w^\top \vect z+ b)
\end{align}
where $\vect w\in\mathbb{R}^d, \vect u\in\mathbb{R}^d, b\in\mathbb{R}$
are parameters and $h(\cdot)$ is a univariate non-linear function with
derivative $h'(\cdot)$. For this family of transformations, the
determinant of the Jacobian matrix can be computed as
\begin{align}
  \det\frac{\partial f}{\partial \vect z}=\det(\vect I+\vect u\psi(\vect z)^\top)=1+\vect u^\top \psi(\vect z)
\end{align}
where $\psi(\vect z)=h'(\vect w^\top \vect z+b)\vect w$. The
computation cost of the determinant is hence reduced from
$\mathcal{O}(d^3)$ to $\mathcal{O}(d)$.

Applying $f$ to $\vect z$ can be viewed as feeding the input variable
to a neural network with only one single hidden unit followed by a
linear output layer which has the same dimention with the input
layer. Obviously, because of the bottleneck caused by the single
hidden unit, the capacity of the family of transformed density is
hence limited.

\section{A NEW TRANSFORMATION UNIT}

In this section, we first propose a direct extension to the above
mentioned planar normalizing flow, and then propose a more general
transformation unit which admitts larger distribution coverage as well
as maintaining linear computation efficiency.

\subsection{Normaling flow with $d$ hidden units}

Instead of having a single hidden unit as suggested in planar flow,
consider $d$ hidden units in the process. We denote the weights
associated with the edges from the input layer to the output layer as
$\vect W$ and the weights from the hidden layer to the output layer
as $\vect U$, and the transformation is defined as
\begin{align}
  f(\vect z)=\vect Uh(\vect W\vect z+\vect b)
\end{align}
The Jacobian matrix of this transformation is ?
\begin{align}
  \frac{\partial f}{\partial \vect z}&=\vect U\mbox{diag}(h'(\vect W\vect z+b))\vect W\\
  \det\frac{\partial f}{\partial \vect z}&=\det(\vect U) \det(\mbox{diag}(h'(\vect W\vect z+b)))\det(\vect W)
  \end{align}

As $\det(\mbox{diag}(h'(\vect W\vect z+\vect b)))$ is linear, the
complexity of computing the above transformation lies in computing
$\det (\vect W)$ and $\det(\vect U)$. Essentialy the planar flow is
restricting that both $\vect W$ and $\vect U$ are just vectors of
length $d$ instead of matrices, however we can relax that assumption
while still maintaining linear complexity of the determinant
computation based on a very simple fact that the determinant of a
triangle matrix is also just the product of the elements on the
diagonal. We call this transformation as triangular flow.

We can stack the triangular flows for multiple layers and construct arbitrarily
complex distributions as desired.

\begin{comment}

\begin{align}
  \frac{\partial f}{\partial \vect z}=\mbox{diag}(h'(\vect W\vect z+b))\vect W\\
  \det\frac{\partial f}{\partial \vect z}=\det(\mbox{diag}(h'(\vect W\vect z+b)))\det(\vect W)
\end{align}

The PDF of $f$ is
\begin{align}
  p(f)=p(\vect z)\left|\det\frac{\partial f}{\partial \vect z}\right|^{-1}\\
    \log p(f)=\log p(\vect z)-\log\left|\det\frac{\partial f}{\partial \vect z}\right|
\end{align}

Given the transformation in bijective
\begin{align}
  \log\left|\det\frac{\partial f}{\partial \vect z}\right|=\log|\det(\mbox{diag}(h'(\vect W\vect z+b)))|+\log|\det(\vect W)|
\end{align}
as long as $\vect W$ is of full rank.

For efficiency, we may requre that computing $\det(W)$ is easy.

\subsection{Fitting Residue}
\begin{align}
    f(\vect z)=\vect z+h(\vect W\vect z+\vect b)
\end{align}
The Jacobian is
\begin{align}
    \frac{\partial f}{\partial \vect z}=\vect I+ \mbox{diag}(h'(\vect W\vect z+b))\vect W
%  \det\frac{\partial f}{\partial \vect z}=\det(\mbox{diag}(h'(\vect W\vect z+b)))\det(\vect W)
\end{align}
\end{comment}

\subsection{Normalizing flow with infinite hidden units}

The above triangular flow improves the coverage of the transformed
probability densities by leveraging the triangular weight matrices
while maintiaining the linear computation of the determinant of the
Jacobian matrix. Though we can stack up multiple layers to model
arbitrarily complicated distributions, the representation power of one
single layer is still limited as we are using only $d$ hidden units
for one flow only to facilitate the computation of the determinant of
the individual weight matrix (otherwise the weight matrix is
non-square hence the determinant is undefined), which might not
necessarily the optimum choice of hidden unit size.

In this section, we do not put an explicit constraints over the number
of hidden units in the flow. Formally, we assume the weight matrix
form the input layer to the hidden layer to be $\vect
W\in\mathbb{R}^{s\times d}$ and the weight matrix from the hidden
layer to be $\vect U\in\mathbb{R}^{d\times s}$. Hence the transformed variable after one flow is
\begin{align}
  \vect z'=f(\vect z)=\vect U h(\vect W\vect z+\vect b)
\end{align}
And the Jacobian matrix is
\begin{align}
    \frac{\partial f}{\partial \vect z}&=\vect U[\mbox{diag}(h'(\vect W\vect z+b))\vect W]
\end{align}
However, its determinant cannot be decomposed as the product of the
individual determinant of three terms as $\vect W$ and $\vect U$ are not necessarily square matrices.

However, in the extreme case, as well to fully exploit the hidden
units for better normalizing, we push the number of hidden units to
its limit , i.e., $s\rightarrow\infty$. Specifically, in this case
\begin{align}
  [f(\vect z)]_k&=\sum_{j=1}^\infty u_{jk} h_j(\vect z)\\
  h_j(\vect z)&=\mbox{tanh}\left(\sum_{i=1}^d w_{ij}\vect z_i+b_j\right), &\mbox{ for }j=1,2,.., \infty
  \end{align}

This essentially defines a Gaussian Process (GP) over each dimension
of $f(\vect z)$ \cite{neal1995bayesian}. To reparameterize, the prior
over all these trasnformation is
\begin{align}
  \pi(f)=\prod_{i=1}^d\mathcal{GP}(f_i;\vect 0,k(\vect z_1, \vect
  z_2))
\end{align}
where we assume the mean function of all GPs are 0 and $k(\cdot,
\cdot)$ denotesthe covariance function evaluated on a pair of inputs
from $\mathbb{R}^d$. Hence each sample from this GP defines a
tranformation function over $\vect z$, and we aim to find the best
$f^*$ such that under that transformation, the density of $f(\vect z)$
best approxmiate the true posterior.

However since GP is a nonparameteric model, we cannot derive the exact
from of $p(f(\vect z))$ by the change of variable theorem, since we
can no longer evaluate analytically the Jacobian of $f$ w.r.t to
$\vect z$. Nevertheless, we don't require to access the analytic form
of Jacobian as we are only interested in its evaluations at the given
inputs $\{\vect z_i\}$. Since $f$ is now random, the corresponding
Jacobian also turns to a random matrix. Moreover, the Jacobian
evaluated at input $\vect z$ can be approximated as $\hat J(\vect z)=\left[ \frac{\partial f(\vect z)_i}{\partial\vect z_j}\right]_{ij}$ where
\begin{align}
  \frac{\partial f(\vect z)_i}{\partial\vect z_j}=\lim_{\Delta\rightarrow 0}\frac{f(\vect z+\Delta \vect e)_i-f(\vect z)_i}{\Delta}
\end{align}
Hence the determinant of the Jacobian can also be approximated. Note
now the determinant is also a random quantity. And so is the KL
divergence from the density of the transformed variable to the true
posterior. Hence we aim to minimize the expected KL divergence loss
w.r.t to this randomness as
\begin{align}
\mathbb{E}\, KL(p(f(\vect z))||p(z|\vect X))
\end{align}

Model can be trained via SGD with the detailed parameter gradient as follows:

\begin{comment}
\begin{align}
  f(\vect z)=\vect L\vect z+\vect K_{\vect z\vect x}\vect
  K^{-1}_{\vect x\vect x}\vect z
\end{align}
where
\begin{align}
  \vect L\vect L^\top=\vect K_{\vect z\vect z}-\vect K\vect K\vect K
  \end{align}
  and for each transform, its corresponding Jacobian is
\begin{align}
\det\frac{\partial f}{\partial \vect z}&=\det(\vect U\mbox{diag}(h'(\vect W\vect z+b))\vect W)
\end{align}
which can be further decomposed as ...
\end{comment}

\section{THEORETICAL ANALYSIS}

\section{EVALUATIONS}

We present the evaluation results of the proposed normalizing methods
with the normalizing flow on both synthetic data sets and real world
Bayesian learning settings.

\subsection{Synthetic data sets}

For the synthetic setting, we manually specify some true (posterior)
distribution and apply the proposed methods as well as baseline
methods to approximate the target distribution. The list of used
synthetic distribution can be found in Table \ref{tab:dis}

\begin{table}
  \centering
  \begin{tabular}{l}
    \toprule
    Potential $U(\vect z)$\\
    \midrule
    1: $\frac{1}{2}\left(\frac{\|\vect z\|-2}{0.4}\right)^2-\log\left(e^{-\frac{1}{2}\left[\frac{\vect z_1-2}{0.6}\right]^2}+e^{-\frac{1}{2}\left[\frac{\vect z_1+2}{0.6}\right]^2}\right)$\\
    2: $\frac{1}{2}\left[\frac{\vect z_2-w_1(\vect z)}{0.4}\right]^2$\\
    3: $-\log\left(e^{-\frac{1}{2}\left[\frac{\vect z_2-w_1(\vect z)}{0.4}\right]^2}+e^{-\frac{1}{2}\left[\frac{\vect z_2-w_1(\vect z)+w_3(\vect z)}{0.35}\right]^2}\right)$\\
    \midrule
    with $w_1(\vect z)=\sin\left(\frac{\pi\vect z_1}{2}\right)$, $w_3(\vect z)=3\sigma\left(\frac{\vect z_1-1}{0.3}\right)$ and\\$\sigma(x)=1/(1+e^{-x})$\\
    \bottomrule
  \end{tabular}
  \end{table}

\subsection{Bayesian Logistic Regression}



